DB3V: A Dialect Dominated Dataset of Bird Vocalisation for Cross-corpus Bird Species Recognition

In ornithology, bird species are known to have variedit's widely acknowledged that bird species display diverse dialects in their calls across different regions. Consequently, computational methods to identify bird species onsolely through their calls face critsignificalnt challenges. There is growing interest in understanding the impact of species-specific dialects on the effectiveness of bird species recognition methods. Despite potential mitigation through the expansion of dialect datasets, the absence of publicly available testing data currently impedes robust benchmarking efforts. This paper presents the Dialect Dominated Dataset of Bird Vocalisation, the first cross-corpus dataset that focuses on dialects in bird vocalisations. The DB3V comprises more than 25 hours of audio recordings from 10 bird species distributed across three distinct regions in the contiguous United States (CONUS). In addition to presenting the dataset, we conduct analyses and establish baseline models for cross-corpus bird recognition. The data and code are publicly available online: https://zenodo.org/records/11544734

==> note.tex <==
North America can be broadly divided into three main geographical regions:


Western Cordillera (100W \~ 130W): This region is characterized by mountain ranges, including the Rocky Mountains and the Coastal Ranges. It extends along the western part of North America.

Interior Plains (90W \~ 100W): The vast and flat area known as the Great Plains lies between the Western Cordillera and the Appalachian Mountains. It is a region of extensive grasslands.

Eastern Highlands (70W \~ 00W): The Appalachian Mountains, running along the eastern part of the continent, form the Eastern Highlands. This region consists of forested mountains and valleys.

Western Cordillera（西部山脉区）: 这个区域位于北美的西部，包括落基山脉和沿海山脉。从经度上来看，你可以将其大致划定在西经100度到西经130度之间。

Interior Plains（内陆平原区）: 这片广阔而平坦的区域位于西部山脉区和阿巴拉契亚山脉之间。从经度上来看，你可以将其大致划定在西经90度到西经100度之间。

Eastern Highlands（东部高原区）: 这个区域主要由阿巴拉契亚山脉组成，位于北美的东部。从经度上来看，你可以将其大致划定在西经70度到西经90度之间。

general approximations:

Western Cordillera: This region, located in the western part of North America and comprising the Rocky Mountains and Coastal Ranges, can be roughly considered to span from around 100 degrees west to 130 degrees west.

Interior Plains: Extending between the Western Cordillera and the Appalachian Mountains, the Interior Plains cover a vast and flat area. In terms of longitude, you can approximate it to span from around 90 degrees west to 100 degrees west.

Eastern Highlands: Positioned in the eastern part of North America and mainly composed of the Appalachian Mountains, this region can be roughly considered to span from around 70 degrees west to 90 degrees west.



气候
Western Cordillera（西部山脉区）: 这个区域通常表现出多样化的气候，具体取决于海拔高度。在较低海拔地区，你可能会遇到干燥的沙漠气候，而在高海拔地区，气候可能更寒冷，甚至有雪。沿海地区可能经历温和的气候，受到海洋影响。

Interior Plains（内陆平原区）: 内陆平原通常具有大陆性气候，夏季可能很炎热，冬季可能很寒冷。由于缺乏大的地形障碍，这个区域的气候受到湿度和大气运动的影响。

Eastern Highlands（东部高原区）: 这个区域通常经历四季分明的温带气候，夏季可能温暖而潮湿，冬季可能寒冷，经常伴随着降雪。阿巴拉契亚山脉可能对气候产生影响，导致东风面相对湿润，而西风面相对较干燥。

Western Cordillera: This region typically exhibits diverse climates, depending on altitude. Lower elevations may experience arid or desert climates, while higher elevations can be colder, with the possibility of snow. Coastal areas might have milder climates influenced by the ocean.

Interior Plains: The interior plains generally have a continental climate with hot summers and cold winters. The absence of significant topographical barriers allows humidity and atmospheric patterns to influence the climate.

Eastern Highlands: The Eastern Highlands usually experience a temperate climate with distinct seasons. Summers can be warm and humid, while winters are often cold with frequent snowfall. The presence of the Appalachian Mountains can impact the climate, creating relatively moist conditions on the windward side and drier conditions on the leeward side.
